Greedy Approximation Algorithms for Active Sequential Hypothesis Testing

In the problem of active sequential hypothesis testing (ASHT), a learner seeks to identify the true hypothesis from among a known set of hypotheses. The learner is given a set of actions and knows the random distribution of the outcome of any action under any true hypothesis. Given a target error $\delta>0$, the goal is to sequentially select the fewest number of actions so as to identify the true hypothesis with probability at least $1 - \delta$. Motivated by applications in which the number of hypotheses or actions is massive (e.g., genomics-based cancer detection), we propose efficient (greedy, in fact) algorithms and provide the first approximation guarantees for ASHT, under two types of adaptivity. Both of our guarantees are independent of the number of actions and logarithmic in the number of hypotheses. We numerically evaluate the performance of our algorithms using both synthetic and real-world DNA mutation data, demonstrating that our algorithms outperform previously proposed heuristic policies by large margins.

==> NIPS_submission/trash.tex <==
\begin{proof}
Let $\tilde\sigma=(a_1,a_2,...)$ be the \xulie\ after the boosting step and fix any true \hypo\ $h$. 
Write $Z(h,g;a_i)=Z_i$, then for any $t\geq 1$, it holds $\log \Lambda(h,g;t)=\sum_{i=1}^t Z_i$.
By definition of cover time, we have $\sum_{i=1}^{\tau(h)} \ho{E}Z_i \geq \alpha \theta$. 
Thus, 
\begin{align}
\ho{P}_h \Big[\log\Lambda\big(h,g;\tau(h)\big)< \frac{1}{2}\alpha\theta\Big]
&=\ho{P}_h\Big[\sum_{i=1}^{\tau(h)} Z_i < \frac{1}{2}\alpha\theta\Big] \notag\\
&\leq \ho{P}_h\Big[|\sum_{i=1}^M Z_i - \sum_{i=1}^{\tau(h)} \ho{E}Z_i| > \frac{1}{2}\sum_i \ho{E}Z_i\Big].\label{eqn:oct13}
\end{align}

To apply Hoeffding's \ineq\ to (\ref{eqn:oct13}), we bound $|Z_i|$ as follows. 
Write $\Delta_i = \mu(h,a_i)-\mu(g,a_i)$, then
\[Z_i = 
\begin{cases}
\log (1+\frac{\Delta_i}{\mu(g,a_i)}), \quad &\text{ w.p. } \mu(h,a_i),\\
\log (1-\frac{\Delta_i}{1-\mu(g,a_i)}), \quad &\text{ w.p. } 1-\mu(h,a_i).
\end{cases}\]
Since $0<\mu_{min}\leq \mu(g,a_i) \leq \mu_{\max}<1$, we have $|Z_i| \leq C|\Delta_i|$
where $C=2\max\{(1-\mu_{max})^{-1},\mu_{min}^{-1}\}$.
By taking $\eps=\frac{1}{2}\sum_{i=1}^{\tau(h)} \ho{E}Z_i$ in Theorem~\ref{thm:hoeffding_ber}, we obtain:
\beqn\label{eqn:oct10}
(\ref{eqn:oct13})\leq \exp\Big(-\Omg\Big(\frac{(\alpha\theta)^2}{\sum_{i=1}^{\tau(h)} \Delta_i^2}\Big)\Big).
\eeqn
We claim that $\alpha\theta \geq \Omg(\sum_{i=1}^{\tau(h)}\Delta_i^2)$. In fact, write $t=CT(f_h^\theta,\sigma)$, where $\sigma$ is the \xulie\ {\bf{before}} boosting. By definition of cover time, \[\sum_{i=1}^{\alpha t} d(h,g;a_i)\geq \alpha\theta \geq \sum_{i=1}^{\alpha(t-1)} d(h,g;a_i).\]

\parag{Fact.} Let $\mu\in (0,1)$, and $d(p||q)$ be the KL-divergence from $Ber(p)$ to $Ber(q)$. Then, $d(\mu+\delta||\mu)\geq \Omg(\delta^2)$ as $\delta\rar 0^+$. 

Hence,
\beqn
\alpha\theta\geq \sum_{i=1}^{\alpha(t-1)}
d(h,g,a_i)\geq \Omg(\sum_{i=1}^{\alpha(t-1)} \Delta_i^2)= \Omg(\sum_{i=1}^{\tau(h)} \Delta_i^2).\notag
\eeqn
It follows that $(\ref{eqn:oct10})\leq \exp(-\Omg(\alpha \theta))$. The proof completes by applying the union bound over all $g\in H\bs \{h\}$.
\end{proof}

\begin{theorem}[Hoeffding Inequality for Bernoulli]\label{thm:hoeffding_ber}
Let $X_i$, $i=1,..,n$, be \indep\ \rv s each supported on $[u_i, \ell_i]$. 
Then for any $\eps>0$, it holds that \[\ho{P}\Big[|\sum_{i=1}^n X_i - \sum_{i=1}^n \ho{E}X_i|\geq \eps\Big]\leq \exp(-\frac{2\eps^2}{\sum_i (\ell_i-u_i)^2}).\]
\end{theorem}


==> old_sections/experiments.tex <==
Since the approximation ratio
that we derived in Section~\ref{sec:adaptive} compares the performance of our algorithm to the optimal algorithm, in this section, we illustrate the relative performance of our proposed greedy algorithm with offline and online heuristic algorithms proposed in \cite{gan2020causal}. We show that our greedy algorithm can be relaxed to the setting where the hypothesis space is continuous without discretization, and the submodular function can be relaxed to be outcome dependent.

We first demonstrate the efficiency of our heuristic algorithm using a synthetic dataset, where the data generating distributions, $\mathbb{P}_{Y,T,Z}$,  were randomly chosen over the unit-7 simplex. We measure the performance of the algorithms in terms of the expected absolute estimation error of ATE. Finally, we validate the performance of the greedy algorithm on a real-world dataset---COSMIC \citep{tate2019cosmic, cosmic2019}---that includes genetic mutations of cancer patients.

% are not necessarily tight, we first perform synthetic experiments to assess the tightness of our bounds. 
% For the purpose of illustration, we focus on binary confounders $Z$ throughout this section, and denote $q_{yt} = P_{Z=1|Y,T}(y,t)$. 
% We first compare the sampling policies in synthetic experiments on randomly chosen distributions $P_{Y,T,Z}$, %chose distributions over $P_{Y,T,Z}$ by sampling uniformly over the 
%unit 7-simplex, 
% measuring both the average and worst-case performance of each sampling policy.
% over these parameters. 
% We then measure the effect of having finite (vs. infinite) confounded data. Finally, we test the performance of OWSP on real-world data taken from a genetic database, COSMIC, that includes genetic mutations of cancer patients
% and other patient characteristics 
% \citep{tate2019cosmic, cosmic2019}.

\subsection{Experiment Setup}

Instead of discretizing the hypothesis space, in this section, we move the problem into a Bayesian setting, where the submodular function $f^h$ is now dependent on the outcome of the test.
Let $\rm{Ber}(y_{yx})$ denote the Bernoulli random variable with mean $q_{yx}$.
% , i.e., $B(q_{yx})$ is the random variable denoting the outcome that we would observe that if we choose to sample an additional data from the group $(y,x)$. 
Since the beta distribution is the conjugate prior for Bernoulli distributions, we initialize a beta distribution for each $\rm{Ber}(q_{yx})$, where the initial $\alpha$ and $\beta$ parameters of the distribution are set to 1. Once more data are revealed, we update the beta distribution. Thus, we calculate $f^h(E)$ as (to be completed after the completion of the algorithm section)

$f^h(E\cup e)$ to be described 

In addition, instead of predefining a discretization for ATE equivalent classes, we update the discretization of ATE equivalent class dynamically. In particular, at each step, we rediscretize the alive ATE equivalent classes into a constant number of classes.

Furthermore, we select one sample at a time in the each iteration, and set $c_e$ to be 1. At each step, we greedily select the group with the highest score to sample from in the next iteration, where the score function is now defined as:
\begin{equation}
  \text{score}(e; E, A) = \int \limits_{j\in L_e(A)} 1 dj + \int \limits_{h\in \pi_A} \frac{f^h (E\cup e) - f^h (E)}{1-f^h (E)}dh. 
\end{equation}



\paragraph{Benchmarks}
We compare our proposed greedy algorithm with two non-adaptive and one adaptive algorithms proposed in \cite{gan2020causal}. Let $x_{yx}$ denote the percentage of data that we are going to select from group $yx$ to deconfound. Then, in the two offline policies, the ratios $x_{yx}$s are fixed a priori. More specifically, they are defined the as follows: 
\begin{itemize}
    \item Natural (NSP): $x_{yx} = a_{yx} = \mathbb{P}_{Y,X}(y,x)$.
    \item Outcome-weighted (OWSP):
    $x_{yx} = \frac{a_{yx}}{2\sum_y a_{yx}} = \mathbb{P}_{Y|X}(y|x)/2$.
\end{itemize}
To sample data according to NSP is  equivalent to sample a new data point according to the distribution $\mathbb{P}_{Y,X,Z}$ and only reveal the corresponding $Z$ value.
The intuition behind OWSP is that we want to allocate half of the sample to treatment ($X=1$), and half to no treatment $(X=0)$, and within each treatment group, we sample proportional to the outcome ($Y=0$ vs. $1$). 

The greedy algorithm proposed by \cite{gan2020causal} is to choose the group that maximizes the expected change in the estimate ATE in each iteration. We will call this greedy algorithm \emph{baseline greedy} (BGSP). Let 
$\hat{q}_{yx}$ denote the estimated $q_{yx}$ according to data using the Maximum Likelihood Estimator (MLE), and let 
$\widehat{\ATE}(q_{yt} = q)$ denote the estimated ATE obtained by updating the estimated ${q}_{yx}$ to $q$ while keeping the rest estimates the same in Equation (\ref{eq:def_ATE}).
The objective of the \emph{baseline greedy} algorithm is given as follows:
$$ \mathbb{E}\left[ \left|\widehat{\ATE}\left(q_{yx} = \frac{n_{yx}\hat{q}_{yx}+\rm{Ber}(\hat{q}_{yx})}{n_{yx}+1} \right) - \widehat{\ATE}(q_{yx}=\hat{q}_{yx}) \right| \right],$$
where $n_{yx}$ denotes the number of samples we have sampled from the group $(Y=y,X=x)$ so far.

To be consistent with the evaluation metric used in \cite{gan2020causal}, in this section, we
We evaluate the performance the our algorithm as well as the benchmark algorithms using $|\widehat{ATE} - ATE|$, where $\widehat{ATE}$ is the estimated ATE obtained by plugging in the estimated $q_{yx}$s into Equation (\ref{eq:def_ATE}).

\subsection{Synthetic Experiments}
In the left of Figure~\ref{fig:online}, we first evaluate our proposed method against the benchmarks over an ensemble of distributions randomly generated from the distribution parameter simplex. The left of Figure~\ref{fig:online} is averaged over 1,300 distribution instances, $\mathbb{P}_{Y,X,Z}$, uniformly drawn from the unit 7-simplex. Each distribution instance is further averaged over 4 replications. The average absolute error was calculated against the number of deconfounded samples in steps of 15 samples. The middle of Figure~\ref{fig:online} compares the average absolute error of our proposed greedy algorithm against that of the \emph{baseline greedy} sampling policy. 


\begin{figure*}[!ht]
    \centering
    \begin{subfigure}
    \centering
    \includegraphics[width=0.28\textwidth]{figures/ACL_130_10_10.png}
    \end{subfigure}
    \begin{subfigure}
    \centering
    \includegraphics[width=0.34\textwidth]{figures/ACL_scatter_1.png}
    \end{subfigure}
    \begin{subfigure}
    \centering
    \includegraphics[width=0.34\textwidth]{figures/ACL_scatter_2.png}
    \end{subfigure}
    % \vspace{-5mm}
    \caption{Performance of online policies (Greedy and new objective) vs. offline policies (NSP and OWSP), assuming infinite confounded data. Left: averaged over 1,300 distributions, each consisting of $10$ replications. Middle and Right:  $50$ distributions, each averaged over 1,000 replications, where the radius of the circle is the same as the variance.}
    \label{fig:online}
\end{figure*}

\subsection{Real-World Experiments}


\begin{figure*}[!ht]
\begin{subfigure}
    \centering
    \includegraphics[width=0.27\textwidth]{figures/cosmic_1.png}
    \end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.35\textwidth]{figures/cosmic_scatter_1.png}
\end{subfigure}
\begin{subfigure}
    \centering
    \includegraphics[width=0.35\textwidth]{figures/cosmic_scatter_2.png}
\end{subfigure}
% \vspace{-5mm}
    \caption{Performance of the four sampling policies on the real-world dataset---COSMIC---assuming infinite confounded data.  $23$ unique (cancer, mutation, age) combinations were extracted from the dataset. Left: averaged over $23$ instances, and each averaged over 3,000 replications. Middle and Right: error comparison at $150$ deconfounded samples. {\color{red} more instances to be added}}
    \label{fig:cosmic}
\end{figure*}

==> old_sections/model.tex <==
We begin by introducing a model that is general enough to capture the problem of active deconfounding for the most common causal models. Our main subject of interest is a probability distribution $(X,Y,Z)$ taking values in $\{0,1\} \times \{0,1\} \times \mathcal{Z}$, where $X$ is meant to encode whether or not the treatment of interest is performed, $Y$ encodes a binary outcome, and $Z$ encodes the relevant confounding variables taking values in some finite set $\mathcal{Z}$. This distribution is unknown to us, and the data we begin with consists of $n$ {\em confounded samples}, each consisting of an independent draw from this distribution, with the value of $Z$ hidden in each row.

Let $\mathbb{P}$ denote the set of all probability distributions over $\{0,1\} \times \{0,1\} \times \mathcal{Z}$. The only other component needed to specify our problem is the {\em average treatment effect ($\ATE$)}, a functional over $\mathbb{P}$ defined in the language of Pearl's do-calculus as 
\begin{align} 
 	\ATE(X,Y,Z)
 	& \equiv \mathsf{E}[Y|\Do(X=1)] - \mathsf{E}[Y|\Do(X=0)] \\
 	& = \mathsf{E}_Z\mathsf{E}[Y|X=1,Z] - \mathsf{E}_Z\mathsf{E}[Y|X=0,Z].\label{eq:def_ATE}
 \end{align}
The specific form of $\ATE$ above is not particularly important. All that matters for the subsequent analysis is that $\ATE$ is bounded and continuous over some parameterization of $\mathbb{P}$.

Our goal is to estimate the $\ATE$ of the unknown distribution generating our data. To do this, we may {\em deconfound} any of the samples of our data, which reveals the value of $Z$ within that row, or equivalently, makes one draw from the conditional distribution $Z|(X=x,Y=y)$ for a given choice of $(x,y) \in \{0,1\}^2$.
Thus, the decision any algorithm must make is of which samples to deconfound. Policies are allowed to be completely adaptive, meaning deconfounding is done one sample at a time, with the results of previously-deconfounded samples potentially affecting future actions. Loosely, we are interested in finding policies which estimate the $\ATE$ using as few deconfounded samples as possible.

We will make two modeling assumptions. The first is that $n$, the number of confounded samples with which we begin, is effectively infinite. Concretely, this means that 
\begin{assumption}
\label{assump:1}
we know exactly the unknown distribution marginalized over $Z$, and 
\end{assumption}
\begin{assumption}
\label{assump:2}
there are always enough samples so that any of the four possible actions in $\{0,1\}^2$ is feasible.
\end{assumption}

The second assumption is that we have a Bayesian prior on the conditional distributions $Z|(X=x,Y=y)$.

Despite its apparent restrictions, the above model in fact captures the salient challenges in a substantially larger family of settings. Indeed, while we will focus on this model alone for the remainder of this paper, the algorithm and analysis in the coming sections immediately apply to the following model extensions/generalizations:
\begin{enumerate}
\item ({\em Finite confounded data}): Our assumption of an infinite quantity of confounded samples is made primarily for ease of exposition. In fact, the assumption can be completely relaxed so long as we have a Bayesian prior on the entire distribution $(X,Y,Z)$.
\item ({\em Collecting additional confounded data}): In a setting with a finite quantity of confounded samples, another possible action could be to collect more confounded samples. This additional action can be incorporated.
\item ({\em Heterogeneous costs}): The current model is implicitly one with homogeneous costs: we can think of having a budget to spend on deconfounding, with a {\em constant} cost of deconfounding each sample. Instead, the costs of the actions can be allowed to vary.
%\item ({\em Alternate causal models}): 
\item discrete confounder? $\implies$ multiple confounders?
\end{enumerate}

\su{what is a good \alg? define}


